Blind Non-Uniform Motion Deblurring using Atrous Spatial Pyramid Deformable Convolution and Deblurring-Reblurring Consistency

Many deep learning based methods are designed to remove non-uniform (spatially variant) motion blur caused by object motion and camera shake without knowing the blur kernel. Some methods directly output the latent sharp image in one stage, while others utilize a multi-stage strategy (\eg multi-scale, multi-patch, or multi-temporal) to gradually restore the sharp image. However, these methods have the following two main issues: 1) The computational cost of multi-stage is high; 2) The same convolution kernel is applied in different regions, which is not an ideal choice for non-uniform blur. Hence, non-uniform motion deblurring is still a challenging and open problem. In this paper, we propose a new architecture which consists of multiple Atrous Spatial Pyramid Deformable Convolution (ASPDC) modules to deblur an image end-to-end with more flexibility. Multiple ASPDC modules implicitly learn the pixel-specific motion with different dilation rates in the same layer to handle movements of different magnitude. To improve the training, we also propose a reblurring network to map the deblurred output back to the blurred input, which constrains the solution space. Our experimental results show that the proposed method outperforms state-of-the-art methods on the benchmark datasets. The code is available at https://github.com/Dong-Huo/ASPDC.

==> tables/tab_comparison_1_2.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
Method & Xu~\cite{xu2013unnatural}    & Sun~\cite{sun2015learning} & Nah~\cite{nah2017deep}   & Kupyn~\cite{kupyn2018deblurgan} & Tao~\cite{tao2018scale}    & Zhang~\cite{zhang2018dynamic} & Kupyn~\cite{kupyn2019deblurgan}        & Aljadaan~\cite{aljadaany2019douglas} \\ \hline
Pub & CVPR'13 & CVPR'15& CVPR'15& CVPR'18& CVPR'18& CVPR'18& ICCV'19&CVPR'19 \\ \hline
PSNR   & 20.30 & 25.31 & 28.49 & 28.70 & 30.26   & 29.19 & 29.55        & 30.35    \\ \hline
SSIM   & 0.741 & 0.851 & 0.917 & 0.927 & 0.934   & 0.931 & 0.934        & \textcolor{red}{0.961}    \\ \hline\hline
Method & Zhang~\cite{zhang2019deep} & Suin~\cite{suin2020spatially}  & Park~\cite{park2019multi}     & Yuan~\cite{yuan2020efficient}  & Purohit~\cite{purohit2020region} & Zhang~\cite{zhang2020deblurring} & Ours & Ours+     \\ \hline
Pub & CVPR'19 & CVPR'20& ECCV'20& CVPR'20& AAAI'20& CVPR'20& & \\ \hline
PSNR   & 31.20 & \textcolor{blue}{32.02} & 31.15  & 29.81 & 31.76   & 31.10 &  31.97      &  \textcolor{red}{32.11}        \\ \hline
SSIM   & 0.945 & 0.953 & 0.945 & 0.937 & 0.953   & 0.942 &  0.957       &  \textcolor{blue}{0.960}        \\ \hline
\end{tabular}
\caption{Quantitative comparison on the GoPro dataset~\cite{nah2017deep}. Ours/Ours+ represents our deblurring network without/with fine-tuning on the kernel generator. The best results are in \textcolor{red}{red} and the second best in \textcolor{blue}{blue}.}
\label{tab:comparison_1}
\end{table*}

==> tables/tab_comparison_3.tex <==
\begin{table}[h]
\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
Method & \multicolumn{2}{c|}{Real-J} & \multicolumn{2}{c|}{Real-R} \\ \cline{2-5} 
                        & PSNR         & SSIM         & PSNR         & SSIM         \\ \hline
Kupyn~\cite{kupyn2019deblurgan}               & 29.69        & 0.870        & 36.44        & 0.935        \\ \hline
Tao~\cite{tao2018scale}                     & 31.38        & 0.909        & 38.65        & 0.965        \\ \hline
Ours                    & 29.80        & 0.933        & 36.23        & 0.974        \\ \hline
Ours+                   &              &              &              &              \\ \hline
\end{tabular}
\caption{Quantitative comparison on Real-J and Real-R datasets~\cite{rim2020real}. Ours/Ours+ represents our deblurring network without/with fine-tuning on the kernel generator. The best results are in \textcolor{red}{red} and the second best in \textcolor{blue}{blue}.}
\label{tab:real}
\end{table}
